Digitizing Paper ECGs at Scale: An Open-Source Algorithm for Clinical Research

Millions of clinical ECGs exist only as paper scans, making them unusable for modern automated diagnostics. We introduce a fully automated, modular framework that converts scanned or photographed ECGs into digital signals, suitable for both clinical and research applications. The framework is validated on 37,191 ECG images with 1,596 collected at Akershus University Hospital, where the algorithm obtains a mean signal-to-noise ratio of 19.65 dB on scanned papers with common artifacts. It is further evaluated on the Emory Paper Digitization ECG Dataset, comprising 35,595 images, including images with perspective distortion, wrinkles, and stains. The model improves on the state-of-the-art in all subcategories. The full software is released as open-source, promoting reproducibility and further development. We hope the software will contribute to unlocking retrospective ECG archives and democratize access to AI-driven diagnostics.

==> perspective_example_images.tex <==
\begin{figure*}[htbp]
    \centering
    \begin{tikzpicture}[node distance=0mm]
        \def\imgwidth{0.32\textwidth}
        \def\sepwidth{0mm}

        % Row 1
        \node[anchor=north west] (img1) at (0, 0) {
            \includegraphics[width=\imgwidth]{figures/perspective/1_raw.png}
        };

        \node[anchor=north west] (img2) at ([xshift=\sepwidth]img1.north east) {
            \includegraphics[width=\imgwidth]{figures/perspective/2_raw.png}
        };

        \node[anchor=north west] (img3) at ([xshift=\sepwidth]img2.north east) {
            \includegraphics[width=\imgwidth]{figures/perspective/3_raw.png}
        };

        % Row 2
        \node[anchor=north west] (img4) at ([yshift=-\sepwidth]img1.south west) {
            \includegraphics[width=\imgwidth]{figures/perspective/1_processed.png}
        };

        \node[anchor=north west] (img5) at ([xshift=\sepwidth]img4.north east) {
            \includegraphics[width=\imgwidth]{figures/perspective/2_processed.png}
        };

        \node[anchor=north west] (img6) at ([xshift=\sepwidth]img5.north east) {
            \includegraphics[width=\imgwidth]{figures/perspective/3_processed.png}
        };
    \end{tikzpicture}
    \caption{Comparison of images before and after perspective correction: the top row shows photos captured using a phone camera, either of a paper or a computer monitor. The bottom row displays the same images after perspective correction, highlighting improved alignment.}
    \label{fig:perspective_grid}
\end{figure*}
